Trials and Tribulations of Chemodynamical Tagging: Investigating the Recovery of Open Clusters in the Gaia DR3-GALAH DR4 Catalog

Chemodynamical tagging has been suggested as a powerful tool to trace stars back to their birth clusters. However, the efficacy of chemodynamical tagging as a means to recover individual stellar clusters is still under debate. In this study, we present a detailed investigation of chemodynamical tagging of open clusters using both dynamical and chemical data from the \textit{Gaia} DR3 and GALAH DR4 surveys, respectively. Using a sample of open clusters and mock field stars, we conduct a bootstrap analysis to evaluate every unique combination of orbital components ($E, J_R, J_\phi, J_Z$) and chemical abundances ([X/Fe] for O, Na, Mg, Al, Si, K, Ca, Sc, Ti, Cr, Mn, Ni, Cu, Y, and Ba) on how well they recover open clusters when used as parameters in the clustering algorithm, HBDSCAN. We find that using primarily dynamical orbital parameters leads to the highest recovery rate of open cluster stars. Nevertheless, even employing the best performing parameter combinations leads to low open cluster recovery rates. We find that, in most cases, chemodynamical tagging of open clusters using blind clustering algorithms is not efficient, which is in line with previous theoretical and observational work. However, we show that the addition of cuts based on metallicity, age, and birth radii in order to reduce the size of the clustering catalog can marginally improve the recovery rate of open clusters.

==> appendices.tex <==
\section{Individual Open Cluster Properties} \label{sec:app}

The common assumption for open clusters is that they are chemically homogeneous, similarly aged, and born in the same position, however, we show that there exists an intrinsic spread in each open cluster. For each open cluster taken from the \citet{Hunt2023} catalog, we plot the GALAH metallicity distributions of all of the member stars. We also plot the distribution of the derived ages and birth radii (see Sections \ref{sec:ages} and \ref{sec:br}, respectively). Additionally, we show the Kiel diagram for each open cluster, which shows if an open cluster is dominated by dwarf stars, giants, or a combination of both. 

Finally, we plot the V-measure scores obtained for each open cluster using the dynamic parameters, $D = E, J_\phi, J_Z, J_R$, and the dynamic parameters with an additional element parameter. The solid areas of each bar plot show the V-measure score associated with our clustering algorithm on the entire \textit{Gaia}-GALAH catalog. The hatched regions show the maximum V-measure score obtained using a combination of metallicity, age, and birth radius restrictions to the catalog. By comparing the maximum V-measure score obtained for each open cluster to the properties of the open clusters, we can determine what properties are important for increasing recovery rates when clustering.

\begin{subfigures}
    \begin{figure}
        \centering
        \includegraphics[width=0.9\linewidth]{figures/summary_plot_ASCC_18.pdf}
        \caption{Characteristics of the open cluster ASCC 18. \textit{Top left}: Distribution of [Fe/H] abundances for member stars in ASCC 18. The mean metallicity from \citet{Hunt2023} is shown as the vertical, dashed line. \textit{Top middle}: Distribution of ages found through stellar evolutionary track fitting, using the YREC, MIST, Dartmouth, and GARSTEC isochrone models. The mean age from \citet{Hunt2023} is shown as the vertical, dashed line. \textit{Top right}: Distribution of birth radii derived using relationship between [Fe/H] and age found in \citet{2022arXiv221204515L}. \textit{Bottom right}: Kiel diagram showing evolutionary stages of member stars of ASCC 18, compared to the GGC. \textit{Bottom right}: Results of how well ASCC 18 is recovered using different parameter combinations. The solid area of each bar represent the V-measure score of clustering the GGC, while the hatched section of the plot represents the best V-measure score achieved using a combination of [Fe/H], age, and birth radii cuts to reduce the size of the GGC.}
        \label{fig:sum_plot_ascc18}
    \end{figure}
    
    \begin{figure}
        \centering
        \includegraphics[width=0.9\linewidth]{figures/summary_plot_ASCC_20.pdf}
        \caption{Same as Figure \ref{fig:sum_plot_ascc18}, but for ASCC 20.}
    \end{figure}
    
    \begin{figure}
        \centering
        \includegraphics[width=0.9\linewidth]{figures/summary_plot_ASCC_21.pdf}
        \caption{Same as Figure \ref{fig:sum_plot_ascc18}, but for ASCC 21.}
    \end{figure}
    
    \begin{figure}
        \centering
        \includegraphics[width=0.9\linewidth]{figures/summary_plot_Blanco_1.pdf}
        \caption{Same as Figure \ref{fig:sum_plot_ascc18}, but for Blanco 1.}
    \end{figure}
    
    \begin{figure}
        \centering
        \includegraphics[width=0.9\linewidth]{figures/summary_plot_Briceno_1.pdf}
        \caption{Same as Figure \ref{fig:sum_plot_ascc18}, but for Briceno 1.}
    \end{figure}
    
    \begin{figure}
        \centering
        \includegraphics[width=0.9\linewidth]{figures/summary_plot_Collinder_261.pdf}
        \caption{Same as Figure \ref{fig:sum_plot_ascc18}, but for Collinder 261.}
    \end{figure}
    
    \begin{figure}
        \centering
        \includegraphics[width=0.9\linewidth]{figures/summary_plot_Collinder_69.pdf}
        \caption{Same as Figure \ref{fig:sum_plot_ascc18}, but for Collinder 69.}
    \end{figure}
    
    \begin{figure}
        \centering
        \includegraphics[width=0.9\linewidth]{figures/summary_plot_IC_4665.pdf}
        \caption{Same as Figure \ref{fig:sum_plot_ascc18}, but for IC 4665.}
    \end{figure}
    
    \begin{figure}
        \centering
        \includegraphics[width=0.9\linewidth]{figures/summary_plot_Mamajek_4.pdf}
        \caption{Same as Figure \ref{fig:sum_plot_ascc18}, but for Mamajek 4.}
    \end{figure}
    
    \begin{figure}
        \centering
        \includegraphics[width=0.9\linewidth]{figures/summary_plot_Melotte_22.pdf}
        \caption{Same as Figure \ref{fig:sum_plot_ascc18}, but for Melotte 22.}
    \end{figure}
    
    \begin{figure}
        \centering
        \includegraphics[width=0.9\linewidth]{figures/summary_plot_Melotte_25.pdf}
        \caption{Same as Figure \ref{fig:sum_plot_ascc18}, but for Melotte 25.}
    \end{figure}
    
    \begin{figure}
        \centering
        \includegraphics[width=0.9\linewidth]{figures/summary_plot_NGC_1817.pdf}
        \caption{Same as Figure \ref{fig:sum_plot_ascc18}, but for NGC 1817.}
    \end{figure}
    
    \begin{figure}
        \centering
        \includegraphics[width=0.9\linewidth]{figures/summary_plot_NGC_1901.pdf}
        \caption{Same as Figure \ref{fig:sum_plot_ascc18}, but for NGC 1901.}
    \end{figure}
    
    \begin{figure}
        \centering
        \includegraphics[width=0.9\linewidth]{figures/summary_plot_NGC_2112.pdf}
        \caption{Same as Figure \ref{fig:sum_plot_ascc18}, but for NGC 2112.}
    \end{figure}
    
    \begin{figure}
        \centering
        \includegraphics[width=0.9\linewidth]{figures/summary_plot_NGC_2204.pdf}
        \caption{Same as Figure \ref{fig:sum_plot_ascc18}, but for NGC 2204.}
    \end{figure}
    
    \begin{figure}
        \centering
        \includegraphics[width=0.9\linewidth]{figures/summary_plot_NGC_2516.pdf}
        \caption{Same as Figure \ref{fig:sum_plot_ascc18}, but for NGC 2516.}
    \end{figure}
    
    \begin{figure}
        \centering
        \includegraphics[width=0.9\linewidth]{figures/summary_plot_NGC_2539.pdf}
        \caption{Same as Figure \ref{fig:sum_plot_ascc18}, but for NGC 2539.}
    \end{figure}
    
    \begin{figure}
        \centering
        \includegraphics[width=0.9\linewidth]{figures/summary_plot_NGC_2632.pdf}
        \caption{Same as Figure \ref{fig:sum_plot_ascc18}, but for NGC 2632.}
    \end{figure}
    
    \begin{figure}
        \centering
        \includegraphics[width=0.9\linewidth]{figures/summary_plot_NGC_2682.pdf}
        \caption{Same as Figure \ref{fig:sum_plot_ascc18}, but for NGC 2682.}
    \end{figure}
    
    \begin{figure}
        \centering
        \includegraphics[width=0.9\linewidth]{figures/summary_plot_NGC_288.pdf}
        \caption{Same as Figure \ref{fig:sum_plot_ascc18}, but for NGC 288.}
    \end{figure}
    
    \begin{figure}
        \centering
        \includegraphics[width=0.9\linewidth]{figures/summary_plot_NGC_362.pdf}
        \caption{Same as Figure \ref{fig:sum_plot_ascc18}, but for NGC 362.}
    \end{figure}
    
    %\begin{figure}
    %    \centering
    %    \includegraphics[width=0.9\linewidth]{figures/summary_plot_NGC_5139.pdf}
    %    \caption{Same as Figure \ref{fig:sum_plot_ascc18}, but for NGC 5139.}
    %    \label{fig:ngc5149}
    %\end{figure}
    
    \begin{figure}
        \centering
        \includegraphics[width=0.9\linewidth]{figures/summary_plot_NGC_6253.pdf}
        \caption{Same as Figure \ref{fig:sum_plot_ascc18}, but for NGC 6253.}
    \end{figure}
    
    \begin{figure}
        \centering
        \includegraphics[width=0.9\linewidth]{figures/summary_plot_NGC_6397.pdf}
        \caption{Same as Figure \ref{fig:sum_plot_ascc18}, but for NGC 6397.}
    \end{figure}
    
    \begin{figure}
        \centering
        \includegraphics[width=0.9\linewidth]{figures/summary_plot_NGC_7099.pdf}
        \caption{Same as Figure \ref{fig:sum_plot_ascc18}, but for NGC 7099.}
    \end{figure}
    
    \begin{figure}
        \centering
        \includegraphics[width=0.9\linewidth]{figures/summary_plot_Ruprecht_147.pdf}
        \caption{Same as Figure \ref{fig:sum_plot_ascc18}, but for Ruprecht 147.}
    \end{figure}
    
    \begin{figure}
        \centering
        \includegraphics[width=0.9\linewidth]{figures/summary_plot_Trumpler_20.pdf}
        \caption{Same as Figure \ref{fig:sum_plot_ascc18}, but for Trumpler 20.}
        \label{fig:trumpler20}
    \end{figure}

\end{subfigures}

\figsetstart

\figsetnum{A}

\figsettitle{Open Cluster Properties and Results}

\figsetgrpstart
\figsetgrpnum{A.1}
\figsetgrptitle{ASCC 18}
\figsetplot{summary_plot_ASCC_18} \label{fig:ascc_18}
\figsetgrpnote{Characteristics of the open cluster ASCC 18. \textit{Top left}: Distribution of [Fe/H] abundances for member stars in ASCC 18. The mean metallicity from the \citet{Hunt2023} sample is shown as the vertical, dashed line. \textit{Top middle}: Distribution of ages found through stellar evolutionary track fitting, using the YREC, MIST, Dartmouth, and GARSTEC isochrone models. The mean age from \citet{Hunt2023} is shown as the vertical, dashed line. \textit{Top right}: Distribution of birth radii derived using relationship between [Fe/H] and age found in \citet{2022arXiv221204515L}. \textit{Bottom right}: Kiel diagram showing evolutionary stages of member stars of ASCC 18, compared to the overall \textit{Gaia}-GALAH sample. \textit{Bottom middle}: Results of how well ASCC 18 is recovered using different parameter combinations. The solid area of each bar represent the V-measure score of clustering the entire \textit{Gaia}-GALAH sample, while the hatched section of the plot represents the best V-measure score achieved using a combination of [Fe/H], age, and birth radii cuts to reduce the size of the \textit{Gaia}-GALAH sample.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{A.2}
\figsetgrptitle{ASCC 20}
\figsetplot{summary_plot_ASCC_20} \label{fig:ascc_20}
\figsetgrpnote{Characteristics of the open cluster ASCC 20. \textit{Top left}: Distribution of [Fe/H] abundances for member stars in ASCC 20. The mean metallicity from the \citet{Hunt2023} sample is shown as the vertical, dashed line. \textit{Top middle}: Distribution of ages found through stellar evolutionary track fitting, using the YREC, MIST, Dartmouth, and GARSTEC isochrone models. The mean age from \citet{Hunt2023} is shown as the vertical, dashed line. \textit{Top right}: Distribution of birth radii derived using relationship between [Fe/H] and age found in \citet{2022arXiv221204515L}. \textit{Bottom right}: Kiel diagram showing evolutionary stages of member stars of ASCC 20, compared to the overall \textit{Gaia}-GALAH sample. \textit{Bottom middle}: Results of how well ASCC 20 is recovered using different parameter combinations. The solid area of each bar represent the V-measure score of clustering the entire \textit{Gaia}-GALAH sample, while the hatched section of the plot represents the best V-measure score achieved using a combination of [Fe/H], age, and birth radii cuts to reduce the size of the \textit{Gaia}-GALAH sample.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{A.3}
\figsetgrptitle{ASCC 21}
\figsetplot{summary_plot_ASCC_21} \label{fig:ascc_21}
\figsetgrpnote{Characteristics of the open cluster ASCC 21. \textit{Top left}: Distribution of [Fe/H] abundances for member stars in ASCC 21. The mean metallicity from the \citet{Hunt2023} sample is shown as the vertical, dashed line. \textit{Top middle}: Distribution of ages found through stellar evolutionary track fitting, using the YREC, MIST, Dartmouth, and GARSTEC isochrone models. The mean age from \citet{Hunt2023} is shown as the vertical, dashed line. \textit{Top right}: Distribution of birth radii derived using relationship between [Fe/H] and age found in \citet{2022arXiv221204515L}. \textit{Bottom right}: Kiel diagram showing evolutionary stages of member stars of ASCC 21, compared to the overall \textit{Gaia}-GALAH sample. \textit{Bottom middle}: Results of how well ASCC 21 is recovered using different parameter combinations. The solid area of each bar represent the V-measure score of clustering the entire \textit{Gaia}-GALAH sample, while the hatched section of the plot represents the best V-measure score achieved using a combination of [Fe/H], age, and birth radii cuts to reduce the size of the \textit{Gaia}-GALAH sample.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{A.4}
\figsetgrptitle{Blanco 1}
\figsetplot{summary_plot_Blanco_1} \label{fig:blanco_1}
\figsetgrpnote{Characteristics of the open cluster Blanco 1. \textit{Top left}: Distribution of [Fe/H] abundances for member stars in Blanco 1. The mean metallicity from the \citet{Hunt2023} sample is shown as the vertical, dashed line. \textit{Top middle}: Distribution of ages found through stellar evolutionary track fitting, using the YREC, MIST, Dartmouth, and GARSTEC isochrone models. The mean age from \citet{Hunt2023} is shown as the vertical, dashed line. \textit{Top right}: Distribution of birth radii derived using relationship between [Fe/H] and age found in \citet{2022arXiv221204515L}. \textit{Bottom right}: Kiel diagram showing evolutionary stages of member stars of Blanco 1, compared to the overall \textit{Gaia}-GALAH sample. \textit{Bottom middle}: Results of how well Blanco 1 is recovered using different parameter combinations. The solid area of each bar represent the V-measure score of clustering the entire \textit{Gaia}-GALAH sample, while the hatched section of the plot represents the best V-measure score achieved using a combination of [Fe/H], age, and birth radii cuts to reduce the size of the \textit{Gaia}-GALAH sample.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{A.5}
\figsetgrptitle{Briceno 1}
\figsetplot{summary_plot_Briceno_1} \label{fig:briceno_1}
\figsetgrpnote{Characteristics of the open cluster Briceno 1. \textit{Top left}: Distribution of [Fe/H] abundances for member stars in Briceno 1. The mean metallicity from the \citet{Hunt2023} sample is shown as the vertical, dashed line. \textit{Top middle}: Distribution of ages found through stellar evolutionary track fitting, using the YREC, MIST, Dartmouth, and GARSTEC isochrone models. The mean age from \citet{Hunt2023} is shown as the vertical, dashed line. \textit{Top right}: Distribution of birth radii derived using relationship between [Fe/H] and age found in \citet{2022arXiv221204515L}. \textit{Bottom right}: Kiel diagram showing evolutionary stages of member stars of Briceno 1, compared to the overall \textit{Gaia}-GALAH sample. \textit{Bottom middle}: Results of how well Briceno 1 is recovered using different parameter combinations. The solid area of each bar represent the V-measure score of clustering the entire \textit{Gaia}-GALAH sample, while the hatched section of the plot represents the best V-measure score achieved using a combination of [Fe/H], age, and birth radii cuts to reduce the size of the \textit{Gaia}-GALAH sample.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{A.6}
\figsetgrptitle{Collinder 261}
\figsetplot{summary_plot_Collinder_261} \label{fig:collinder_261}
\figsetgrpnote{Characteristics of the open cluster Collinder 261. \textit{Top left}: Distribution of [Fe/H] abundances for member stars in Collinder 261. The mean metallicity from the \citet{Hunt2023} sample is shown as the vertical, dashed line. \textit{Top middle}: Distribution of ages found through stellar evolutionary track fitting, using the YREC, MIST, Dartmouth, and GARSTEC isochrone models. The mean age from \citet{Hunt2023} is shown as the vertical, dashed line. \textit{Top right}: Distribution of birth radii derived using relationship between [Fe/H] and age found in \citet{2022arXiv221204515L}. \textit{Bottom right}: Kiel diagram showing evolutionary stages of member stars of Collinder 261, compared to the overall \textit{Gaia}-GALAH sample. \textit{Bottom middle}: Results of how well Collinder 261 is recovered using different parameter combinations. The solid area of each bar represent the V-measure score of clustering the entire \textit{Gaia}-GALAH sample, while the hatched section of the plot represents the best V-measure score achieved using a combination of [Fe/H], age, and birth radii cuts to reduce the size of the \textit{Gaia}-GALAH sample.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{A.7}
\figsetgrptitle{Collinder 69}
\figsetplot{summary_plot_Collinder_69} \label{fig:collinder_69}
\figsetgrpnote{Characteristics of the open cluster Collinder 69. \textit{Top left}: Distribution of [Fe/H] abundances for member stars in Collinder 69. The mean metallicity from the \citet{Hunt2023} sample is shown as the vertical, dashed line. \textit{Top middle}: Distribution of ages found through stellar evolutionary track fitting, using the YREC, MIST, Dartmouth, and GARSTEC isochrone models. The mean age from \citet{Hunt2023} is shown as the vertical, dashed line. \textit{Top right}: Distribution of birth radii derived using relationship between [Fe/H] and age found in \citet{2022arXiv221204515L}. \textit{Bottom right}: Kiel diagram showing evolutionary stages of member stars of Collinder 69, compared to the overall \textit{Gaia}-GALAH sample. \textit{Bottom middle}: Results of how well Collinder 69 is recovered using different parameter combinations. The solid area of each bar represent the V-measure score of clustering the entire \textit{Gaia}-GALAH sample, while the hatched section of the plot represents the best V-measure score achieved using a combination of [Fe/H], age, and birth radii cuts to reduce the size of the \textit{Gaia}-GALAH sample.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{A.8}
\figsetgrptitle{IC 4665}
\figsetplot{summary_plot_IC_4665} \label{fig:IC_4665}
\figsetgrpnote{Characteristics of the open cluster IC 4665. \textit{Top left}: Distribution of [Fe/H] abundances for member stars in IC 4665. The mean metallicity from the \citet{Hunt2023} sample is shown as the vertical, dashed line. \textit{Top middle}: Distribution of ages found through stellar evolutionary track fitting, using the YREC, MIST, Dartmouth, and GARSTEC isochrone models. The mean age from \citet{Hunt2023} is shown as the vertical, dashed line. \textit{Top right}: Distribution of birth radii derived using relationship between [Fe/H] and age found in \citet{2022arXiv221204515L}. \textit{Bottom right}: Kiel diagram showing evolutionary stages of member stars of IC 4665, compared to the overall \textit{Gaia}-GALAH sample. \textit{Bottom middle}: Results of how well IC 4665 is recovered using different parameter combinations. The solid area of each bar represent the V-measure score of clustering the entire \textit{Gaia}-GALAH sample, while the hatched section of the plot represents the best V-measure score achieved using a combination of [Fe/H], age, and birth radii cuts to reduce the size of the \textit{Gaia}-GALAH sample.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{A.9}
\figsetgrptitle{Mamajek 4}
\figsetplot{summary_plot_Mamajek_4} \label{fig:mamajek_4}
\figsetgrpnote{Characteristics of the open cluster Mamajek 4. \textit{Top left}: Distribution of [Fe/H] abundances for member stars in Mamajek 4. The mean metallicity from the \citet{Hunt2023} sample is shown as the vertical, dashed line. \textit{Top middle}: Distribution of ages found through stellar evolutionary track fitting, using the YREC, MIST, Dartmouth, and GARSTEC isochrone models. The mean age from \citet{Hunt2023} is shown as the vertical, dashed line. \textit{Top right}: Distribution of birth radii derived using relationship between [Fe/H] and age found in \citet{2022arXiv221204515L}. \textit{Bottom right}: Kiel diagram showing evolutionary stages of member stars of Mamajek 4, compared to the overall \textit{Gaia}-GALAH sample. \textit{Bottom middle}: Results of how well Mamajek 4 is recovered using different parameter combinations. The solid area of each bar represent the V-measure score of clustering the entire \textit{Gaia}-GALAH sample, while the hatched section of the plot represents the best V-measure score achieved using a combination of [Fe/H], age, and birth radii cuts to reduce the size of the \textit{Gaia}-GALAH sample.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{A.10}
\figsetgrptitle{Melotte 22}
\figsetplot{summary_plot_Melotte_22} \label{fig:melotte_22}
\figsetgrpnote{Characteristics of the open cluster Melotte 22. \textit{Top left}: Distribution of [Fe/H] abundances for member stars in Melotte 22. The mean metallicity from the \citet{Hunt2023} sample is shown as the vertical, dashed line. \textit{Top middle}: Distribution of ages found through stellar evolutionary track fitting, using the YREC, MIST, Dartmouth, and GARSTEC isochrone models. The mean age from \citet{Hunt2023} is shown as the vertical, dashed line. \textit{Top right}: Distribution of birth radii derived using relationship between [Fe/H] and age found in \citet{2022arXiv221204515L}. \textit{Bottom right}: Kiel diagram showing evolutionary stages of member stars of Melotte 22, compared to the overall \textit{Gaia}-GALAH sample. \textit{Bottom middle}: Results of how well Melotte 22 is recovered using different parameter combinations. The solid area of each bar represent the V-measure score of clustering the entire \textit{Gaia}-GALAH sample, while the hatched section of the plot represents the best V-measure score achieved using a combination of [Fe/H], age, and birth radii cuts to reduce the size of the \textit{Gaia}-GALAH sample.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{A.11}
\figsetgrptitle{Melotte 25}
\figsetplot{summary_plot_Melotte_25} \label{fig:melotte_25}
\figsetgrpnote{Characteristics of the open cluster Melotte 25. \textit{Top left}: Distribution of [Fe/H] abundances for member stars in Melotte 25. The mean metallicity from the \citet{Hunt2023} sample is shown as the vertical, dashed line. \textit{Top middle}: Distribution of ages found through stellar evolutionary track fitting, using the YREC, MIST, Dartmouth, and GARSTEC isochrone models. The mean age from \citet{Hunt2023} is shown as the vertical, dashed line. \textit{Top right}: Distribution of birth radii derived using relationship between [Fe/H] and age found in \citet{2022arXiv221204515L}. \textit{Bottom right}: Kiel diagram showing evolutionary stages of member stars of Melotte 25, compared to the overall \textit{Gaia}-GALAH sample. \textit{Bottom middle}: Results of how well Melotte 25 is recovered using different parameter combinations. The solid area of each bar represent the V-measure score of clustering the entire \textit{Gaia}-GALAH sample, while the hatched section of the plot represents the best V-measure score achieved using a combination of [Fe/H], age, and birth radii cuts to reduce the size of the \textit{Gaia}-GALAH sample.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{A.12}
\figsetgrptitle{NGC 1817}
\figsetplot{summary_plot_NGC_1817} \label{fig:ngc_1817}
\figsetgrpnote{Characteristics of the open cluster NGC 1817. \textit{Top left}: Distribution of [Fe/H] abundances for member stars in NGC 1817. The mean metallicity from the \citet{Hunt2023} sample is shown as the vertical, dashed line. \textit{Top middle}: Distribution of ages found through stellar evolutionary track fitting, using the YREC, MIST, Dartmouth, and GARSTEC isochrone models. The mean age from \citet{Hunt2023} is shown as the vertical, dashed line. \textit{Top right}: Distribution of birth radii derived using relationship between [Fe/H] and age found in \citet{2022arXiv221204515L}. \textit{Bottom right}: Kiel diagram showing evolutionary stages of member stars of NGC 1817, compared to the overall \textit{Gaia}-GALAH sample. \textit{Bottom middle}: Results of how well NGC 1817 is recovered using different parameter combinations. The solid area of each bar represent the V-measure score of clustering the entire \textit{Gaia}-GALAH sample, while the hatched section of the plot represents the best V-measure score achieved using a combination of [Fe/H], age, and birth radii cuts to reduce the size of the \textit{Gaia}-GALAH sample.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{A.13}
\figsetgrptitle{NGC 1901}
\figsetplot{summary_plot_NGC_1901} \label{fig:ngc_1901}
\figsetgrpnote{Characteristics of the open cluster NGC 1901. \textit{Top left}: Distribution of [Fe/H] abundances for member stars in NGC 1901. The mean metallicity from the \citet{Hunt2023} sample is shown as the vertical, dashed line. \textit{Top middle}: Distribution of ages found through stellar evolutionary track fitting, using the YREC, MIST, Dartmouth, and GARSTEC isochrone models. The mean age from \citet{Hunt2023} is shown as the vertical, dashed line. \textit{Top right}: Distribution of birth radii derived using relationship between [Fe/H] and age found in \citet{2022arXiv221204515L}. \textit{Bottom right}: Kiel diagram showing evolutionary stages of member stars of NGC 1901, compared to the overall \textit{Gaia}-GALAH sample. \textit{Bottom middle}: Results of how well NGC 1901 is recovered using different parameter combinations. The solid area of each bar represent the V-measure score of clustering the entire \textit{Gaia}-GALAH sample, while the hatched section of the plot represents the best V-measure score achieved using a combination of [Fe/H], age, and birth radii cuts to reduce the size of the \textit{Gaia}-GALAH sample.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{A.14}
\figsetgrptitle{NGC 2112}
\figsetplot{summary_plot_NGC_2112} \label{fig:ngc_2112}
\figsetgrpnote{Characteristics of the open cluster NGC 2112. \textit{Top left}: Distribution of [Fe/H] abundances for member stars in NGC 2112. The mean metallicity from the \citet{Hunt2023} sample is shown as the vertical, dashed line. \textit{Top middle}: Distribution of ages found through stellar evolutionary track fitting, using the YREC, MIST, Dartmouth, and GARSTEC isochrone models. The mean age from \citet{Hunt2023} is shown as the vertical, dashed line. \textit{Top right}: Distribution of birth radii derived using relationship between [Fe/H] and age found in \citet{2022arXiv221204515L}. \textit{Bottom right}: Kiel diagram showing evolutionary stages of member stars of NGC 2112, compared to the overall \textit{Gaia}-GALAH sample. \textit{Bottom middle}: Results of how well NGC 2112 is recovered using different parameter combinations. The solid area of each bar represent the V-measure score of clustering the entire \textit{Gaia}-GALAH sample, while the hatched section of the plot represents the best V-measure score achieved using a combination of [Fe/H], age, and birth radii cuts to reduce the size of the \textit{Gaia}-GALAH sample.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{A.15}
\figsetgrptitle{NGC 2204}
\figsetplot{summary_plot_NGC_2204} \label{fig:ngc_2204}
\figsetgrpnote{Characteristics of the open cluster NGC 2204. \textit{Top left}: Distribution of [Fe/H] abundances for member stars in NGC 2204. The mean metallicity from the \citet{Hunt2023} sample is shown as the vertical, dashed line. \textit{Top middle}: Distribution of ages found through stellar evolutionary track fitting, using the YREC, MIST, Dartmouth, and GARSTEC isochrone models. The mean age from \citet{Hunt2023} is shown as the vertical, dashed line. \textit{Top right}: Distribution of birth radii derived using relationship between [Fe/H] and age found in \citet{2022arXiv221204515L}. \textit{Bottom right}: Kiel diagram showing evolutionary stages of member stars of NGC 2204, compared to the overall \textit{Gaia}-GALAH sample. \textit{Bottom middle}: Results of how well NGC 2204 is recovered using different parameter combinations. The solid area of each bar represent the V-measure score of clustering the entire \textit{Gaia}-GALAH sample, while the hatched section of the plot represents the best V-measure score achieved using a combination of [Fe/H], age, and birth radii cuts to reduce the size of the \textit{Gaia}-GALAH sample.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{A.16}
\figsetgrptitle{NGC 2516}
\figsetplot{summary_plot_NGC_2516} \label{fig:ngc_2516}
\figsetgrpnote{Characteristics of the open cluster NGC 2516. \textit{Top left}: Distribution of [Fe/H] abundances for member stars in NGC 2516. The mean metallicity from the \citet{Hunt2023} sample is shown as the vertical, dashed line. \textit{Top middle}: Distribution of ages found through stellar evolutionary track fitting, using the YREC, MIST, Dartmouth, and GARSTEC isochrone models. The mean age from \citet{Hunt2023} is shown as the vertical, dashed line. \textit{Top right}: Distribution of birth radii derived using relationship between [Fe/H] and age found in \citet{2022arXiv221204515L}. \textit{Bottom right}: Kiel diagram showing evolutionary stages of member stars of NGC 2516, compared to the overall \textit{Gaia}-GALAH sample. \textit{Bottom middle}: Results of how well NGC 2516 is recovered using different parameter combinations. The solid area of each bar represent the V-measure score of clustering the entire \textit{Gaia}-GALAH sample, while the hatched section of the plot represents the best V-measure score achieved using a combination of [Fe/H], age, and birth radii cuts to reduce the size of the \textit{Gaia}-GALAH sample.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{A.17}
\figsetgrptitle{NGC 2539}
\figsetplot{summary_plot_NGC_2539} \label{fig:ngc_2539}
\figsetgrpnote{Characteristics of the open cluster NGC 2539. \textit{Top left}: Distribution of [Fe/H] abundances for member stars in NGC 2539. The mean metallicity from the \citet{Hunt2023} sample is shown as the vertical, dashed line. \textit{Top middle}: Distribution of ages found through stellar evolutionary track fitting, using the YREC, MIST, Dartmouth, and GARSTEC isochrone models. The mean age from \citet{Hunt2023} is shown as the vertical, dashed line. \textit{Top right}: Distribution of birth radii derived using relationship between [Fe/H] and age found in \citet{2022arXiv221204515L}. \textit{Bottom right}: Kiel diagram showing evolutionary stages of member stars of NGC 2539, compared to the overall \textit{Gaia}-GALAH sample. \textit{Bottom middle}: Results of how well NGC 2539 is recovered using different parameter combinations. The solid area of each bar represent the V-measure score of clustering the entire \textit{Gaia}-GALAH sample, while the hatched section of the plot represents the best V-measure score achieved using a combination of [Fe/H], age, and birth radii cuts to reduce the size of the \textit{Gaia}-GALAH sample.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{A.18}
\figsetgrptitle{NGC 2632}
\figsetplot{summary_plot_NGC_2632} \label{fig:ngc_2632}
\figsetgrpnote{Characteristics of the open cluster NGC 2632. \textit{Top left}: Distribution of [Fe/H] abundances for member stars in NGC 2632. The mean metallicity from the \citet{Hunt2023} sample is shown as the vertical, dashed line. \textit{Top middle}: Distribution of ages found through stellar evolutionary track fitting, using the YREC, MIST, Dartmouth, and GARSTEC isochrone models. The mean age from \citet{Hunt2023} is shown as the vertical, dashed line. \textit{Top right}: Distribution of birth radii derived using relationship between [Fe/H] and age found in \citet{2022arXiv221204515L}. \textit{Bottom right}: Kiel diagram showing evolutionary stages of member stars of NGC 2632, compared to the overall \textit{Gaia}-GALAH sample. \textit{Bottom middle}: Results of how well NGC 2632 is recovered using different parameter combinations. The solid area of each bar represent the V-measure score of clustering the entire \textit{Gaia}-GALAH sample, while the hatched section of the plot represents the best V-measure score achieved using a combination of [Fe/H], age, and birth radii cuts to reduce the size of the \textit{Gaia}-GALAH sample.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{A.19}
\figsetgrptitle{NGC 2682}
\figsetplot{summary_plot_NGC_2682} \label{fig:ngc_2682}
\figsetgrpnote{Characteristics of the open cluster NGC 2682. \textit{Top left}: Distribution of [Fe/H] abundances for member stars in NGC 2682. The mean metallicity from the \citet{Hunt2023} sample is shown as the vertical, dashed line. \textit{Top middle}: Distribution of ages found through stellar evolutionary track fitting, using the YREC, MIST, Dartmouth, and GARSTEC isochrone models. The mean age from \citet{Hunt2023} is shown as the vertical, dashed line. \textit{Top right}: Distribution of birth radii derived using relationship between [Fe/H] and age found in \citet{2022arXiv221204515L}. \textit{Bottom right}: Kiel diagram showing evolutionary stages of member stars of NGC 2682, compared to the overall \textit{Gaia}-GALAH sample. \textit{Bottom middle}: Results of how well NGC 2682 is recovered using different parameter combinations. The solid area of each bar represent the V-measure score of clustering the entire \textit{Gaia}-GALAH sample, while the hatched section of the plot represents the best V-measure score achieved using a combination of [Fe/H], age, and birth radii cuts to reduce the size of the \textit{Gaia}-GALAH sample.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{A.20}
\figsetgrptitle{NGC 288}
\figsetplot{summary_plot_NGC_288} \label{fig:ngc_288}
\figsetgrpnote{Characteristics of the open cluster NGC 288. \textit{Top left}: Distribution of [Fe/H] abundances for member stars in NGC 288. The mean metallicity from the \citet{Hunt2023} sample is shown as the vertical, dashed line. \textit{Top middle}: Distribution of ages found through stellar evolutionary track fitting, using the YREC, MIST, Dartmouth, and GARSTEC isochrone models. The mean age from \citet{Hunt2023} is shown as the vertical, dashed line. \textit{Top right}: Distribution of birth radii derived using relationship between [Fe/H] and age found in \citet{2022arXiv221204515L}. \textit{Bottom right}: Kiel diagram showing evolutionary stages of member stars of NGC 288, compared to the overall \textit{Gaia}-GALAH sample. \textit{Bottom middle}: Results of how well NGC 288 is recovered using different parameter combinations. The solid area of each bar represent the V-measure score of clustering the entire \textit{Gaia}-GALAH sample, while the hatched section of the plot represents the best V-measure score achieved using a combination of [Fe/H], age, and birth radii cuts to reduce the size of the \textit{Gaia}-GALAH sample.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{A.21}
\figsetgrptitle{NGC 362}
\figsetplot{summary_plot_NGC_362} \label{fig:ngc_362}
\figsetgrpnote{Characteristics of the open cluster NGC 362. \textit{Top left}: Distribution of [Fe/H] abundances for member stars in NGC 362. The mean metallicity from the \citet{Hunt2023} sample is shown as the vertical, dashed line. \textit{Top middle}: Distribution of ages found through stellar evolutionary track fitting, using the YREC, MIST, Dartmouth, and GARSTEC isochrone models. The mean age from \citet{Hunt2023} is shown as the vertical, dashed line. \textit{Top right}: Distribution of birth radii derived using relationship between [Fe/H] and age found in \citet{2022arXiv221204515L}. \textit{Bottom right}: Kiel diagram showing evolutionary stages of member stars of NGC 362, compared to the overall \textit{Gaia}-GALAH sample. \textit{Bottom middle}: Results of how well NGC 362 is recovered using different parameter combinations. The solid area of each bar represent the V-measure score of clustering the entire \textit{Gaia}-GALAH sample, while the hatched section of the plot represents the best V-measure score achieved using a combination of [Fe/H], age, and birth radii cuts to reduce the size of the \textit{Gaia}-GALAH sample.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{A.22}
\figsetgrptitle{NGC 5139}
\figsetplot{summary_plot_NGC_5139} \label{fig:ngc_5139}
\figsetgrpnote{Characteristics of the open cluster NGC 5139. \textit{Top left}: Distribution of [Fe/H] abundances for member stars in NGC 5139. The mean metallicity from the \citet{Hunt2023} sample is shown as the vertical, dashed line. \textit{Top middle}: Distribution of ages found through stellar evolutionary track fitting, using the YREC, MIST, Dartmouth, and GARSTEC isochrone models. The mean age from \citet{Hunt2023} is shown as the vertical, dashed line. \textit{Top right}: Distribution of birth radii derived using relationship between [Fe/H] and age found in \citet{2022arXiv221204515L}. \textit{Bottom right}: Kiel diagram showing evolutionary stages of member stars of NGC 5139, compared to the overall \textit{Gaia}-GALAH sample. \textit{Bottom middle}: Results of how well NGC 5139 is recovered using different parameter combinations. The solid area of each bar represent the V-measure score of clustering the entire \textit{Gaia}-GALAH sample, while the hatched section of the plot represents the best V-measure score achieved using a combination of [Fe/H], age, and birth radii cuts to reduce the size of the \textit{Gaia}-GALAH sample.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{A.23}
\figsetgrptitle{NGC 6253}
\figsetplot{summary_plot_NGC_6253} \label{fig:ngc_6253}
\figsetgrpnote{Characteristics of the open cluster NGC 6253. \textit{Top left}: Distribution of [Fe/H] abundances for member stars in NGC 6253. The mean metallicity from the \citet{Hunt2023} sample is shown as the vertical, dashed line. \textit{Top middle}: Distribution of ages found through stellar evolutionary track fitting, using the YREC, MIST, Dartmouth, and GARSTEC isochrone models. The mean age from \citet{Hunt2023} is shown as the vertical, dashed line. \textit{Top right}: Distribution of birth radii derived using relationship between [Fe/H] and age found in \citet{2022arXiv221204515L}. \textit{Bottom right}: Kiel diagram showing evolutionary stages of member stars of NGC 6253, compared to the overall \textit{Gaia}-GALAH sample. \textit{Bottom middle}: Results of how well NGC 6253 is recovered using different parameter combinations. The solid area of each bar represent the V-measure score of clustering the entire \textit{Gaia}-GALAH sample, while the hatched section of the plot represents the best V-measure score achieved using a combination of [Fe/H], age, and birth radii cuts to reduce the size of the \textit{Gaia}-GALAH sample.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{A.24}
\figsetgrptitle{NGC 6397}
\figsetplot{summary_plot_NGC_6397} \label{fig:ngc_6397}
\figsetgrpnote{Characteristics of the open cluster NGC 6397. \textit{Top left}: Distribution of [Fe/H] abundances for member stars in NGC 6397. The mean metallicity from the \citet{Hunt2023} sample is shown as the vertical, dashed line. \textit{Top middle}: Distribution of ages found through stellar evolutionary track fitting, using the YREC, MIST, Dartmouth, and GARSTEC isochrone models. The mean age from \citet{Hunt2023} is shown as the vertical, dashed line. \textit{Top right}: Distribution of birth radii derived using relationship between [Fe/H] and age found in \citet{2022arXiv221204515L}. \textit{Bottom right}: Kiel diagram showing evolutionary stages of member stars of NGC 6397, compared to the overall \textit{Gaia}-GALAH sample. \textit{Bottom middle}: Results of how well NGC 6397 is recovered using different parameter combinations. The solid area of each bar represent the V-measure score of clustering the entire \textit{Gaia}-GALAH sample, while the hatched section of the plot represents the best V-measure score achieved using a combination of [Fe/H], age, and birth radii cuts to reduce the size of the \textit{Gaia}-GALAH sample.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{A.25}
\figsetgrptitle{NGC 7099}
\figsetplot{summary_plot_NGC_7099} \label{fig:ngc_7099}
\figsetgrpnote{Characteristics of the open cluster NGC 7099. \textit{Top left}: Distribution of [Fe/H] abundances for member stars in NGC 7099. The mean metallicity from the \citet{Hunt2023} sample is shown as the vertical, dashed line. \textit{Top middle}: Distribution of ages found through stellar evolutionary track fitting, using the YREC, MIST, Dartmouth, and GARSTEC isochrone models. The mean age from \citet{Hunt2023} is shown as the vertical, dashed line. \textit{Top right}: Distribution of birth radii derived using relationship between [Fe/H] and age found in \citet{2022arXiv221204515L}. \textit{Bottom right}: Kiel diagram showing evolutionary stages of member stars of NGC 7099, compared to the overall \textit{Gaia}-GALAH sample. \textit{Bottom middle}: Results of how well NGC 7099 is recovered using different parameter combinations. The solid area of each bar represent the V-measure score of clustering the entire \textit{Gaia}-GALAH sample, while the hatched section of the plot represents the best V-measure score achieved using a combination of [Fe/H], age, and birth radii cuts to reduce the size of the \textit{Gaia}-GALAH sample.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{A.26}
\figsetgrptitle{Ruprecht 147}
\figsetplot{summary_plot_Ruprecht_147} \label{fig:ruprecht_147}
\figsetgrpnote{Characteristics of the open cluster Ruprecht 147. \textit{Top left}: Distribution of [Fe/H] abundances for member stars in Ruprecht 147. The mean metallicity from the \citet{Hunt2023} sample is shown as the vertical, dashed line. \textit{Top middle}: Distribution of ages found through stellar evolutionary track fitting, using the YREC, MIST, Dartmouth, and GARSTEC isochrone models. The mean age from \citet{Hunt2023} is shown as the vertical, dashed line. \textit{Top right}: Distribution of birth radii derived using relationship between [Fe/H] and age found in \citet{2022arXiv221204515L}. \textit{Bottom right}: Kiel diagram showing evolutionary stages of member stars of Ruprecht 147, compared to the overall \textit{Gaia}-GALAH sample. \textit{Bottom middle}: Results of how well Ruprecht 147 is recovered using different parameter combinations. The solid area of each bar represent the V-measure score of clustering the entire \textit{Gaia}-GALAH sample, while the hatched section of the plot represents the best V-measure score achieved using a combination of [Fe/H], age, and birth radii cuts to reduce the size of the \textit{Gaia}-GALAH sample.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{A.27}
\figsetgrptitle{Trumpler 20}
\figsetplot{summary_plot_Trumpler_20} \label{fig:trumpler_20}
\figsetgrpnote{Characteristics of the open cluster Trumpler 20. \textit{Top left}: Distribution of [Fe/H] abundances for member stars in Trumpler 20. The mean metallicity from the \citet{Hunt2023} sample is shown as the vertical, dashed line. \textit{Top middle}: Distribution of ages found through stellar evolutionary track fitting, using the YREC, MIST, Dartmouth, and GARSTEC isochrone models. The mean age from \citet{Hunt2023} is shown as the vertical, dashed line. \textit{Top right}: Distribution of birth radii derived using relationship between [Fe/H] and age found in \citet{2022arXiv221204515L}. \textit{Bottom right}: Kiel diagram showing evolutionary stages of member stars of Trumpler 20, compared to the overall \textit{Gaia}-GALAH sample. \textit{Bottom middle}: Results of how well Trumpler 20 is recovered using different parameter combinations. The solid area of each bar represent the V-measure score of clustering the entire \textit{Gaia}-GALAH sample, while the hatched section of the plot represents the best V-measure score achieved using a combination of [Fe/H], age, and birth radii cuts to reduce the size of the \textit{Gaia}-GALAH sample.}
\figsetgrpend

\figsetend

\section{Individual [Fe/H], Age, and Birth Radius cuts to the \textit{Gaia}-GALAH Catalog} \label{sec:app2}

\begin{figure*}
    \centering
    \includegraphics[width=\linewidth]{figures/vmeas_heatmap_feh_cut.pdf}
    \caption{Same as Figure \ref{fig:heatmap}, except a [Fe/H] cut of $\pm$0.5 dex has been applied to the \textit{Gaia}-GALAH catalog centered on each open cluster.}
    \label{fig:heatmap_feh}
\end{figure*}

\begin{figure*}
    \centering
    \includegraphics[width=\linewidth]{figures/vmeas_heatmap_age_cut.pdf}
    \caption{Same as Figure \ref{fig:heatmap}, except an age cut of $\pm$6 Gyr has been applied to the \textit{Gaia}-GALAH catalog centered on each open cluster.}
    \label{fig:heatmap_age}
\end{figure*}

\begin{figure*}
    \centering
    \includegraphics[width=\linewidth]{figures/vmeas_heatmap_rb_cut.pdf}
    \caption{Same as Figure \ref{fig:heatmap}, except a birth radius cut of $\pm$6 kpc has been applied to the \textit{Gaia}-GALAH catalog centered on each open cluster.}
    \label{fig:heatmap_rb}
\end{figure*}
